A Robust Utility Learning Framework via Inverse Optimization

In many smart infrastructure applications flexibility in achieving sustainability goals can be gained by engaging end-users. However, these users often have heterogeneous preferences that are unknown to the decision-maker tasked with improving operational efficiency. Modeling user interaction as a continuous game between non-cooperative players, we propose a robust parametric utility learning framework that employs constrained feasible generalized least squares estimation with heteroskedastic inference. To improve forecasting performance, we extend the robust utility learning scheme by employing bootstrapping with bagging, bumping, and gradient boosting ensemble methods. Moreover, we estimate the noise covariance which provides approximated correlations between players which we leverage to develop a novel correlated utility learning framework. We apply the proposed methods both to a toy example arising from Bertrand-Nash competition between two firms as well as to data from a social game experiment designed to encourage energy efficient behavior amongst smart building occupants. Using occupant voting data for shared resources such as lighting, we simulate the game defined by the estimated utility functions to demonstrate the performance of the proposed methods.

==> corr_game.tex <==
%In this section, we describe how we leverage learned correlations between
%agents to \emph{boost} our estimators. In particular, we add a second step to the
%estimation procedure. In this step, we craft a new game in
%which agents' utilities are composed of their original estimated utility plus
%some combination of other agents' utilities weighted by the estimated
%correlation between agents.

When the correlations between agents are positive, we are creating what we refer to as \emph{psuedo-coalitions} since
players are not \emph{explicitly} agreeing to collude in the game but rather are doing
so \emph{implicitly}. The degree of \emph{coalition} is discovered by the robust
utility learning process through estimating the empirical
covariance \textcolor{blue!50!black}{\textbf{$\hat{C}_{\beta}$}}, i.e.~asymptotic approximation of the covariance matrix---of
$\hat{\beta}^{\ast}_{est}$ where we use the notation
$\hat{\beta}^{\ast}_{est}$ to abstractly denote the estimator derived from whichever
of the methods described in the previous section is employed. 
On the other hand, when the correlations between agents are negative, by
combining their utilities we aim to take advantage of active voters' richer data
sets in predicting the behavior of agents with less variation and frequency in
their voting record.
%We propose  to take into account the correlations between agents by
%adding a second step to the estimation procedure in which we adjust the learned
%utilities based on the correlation information we extract in the first step.

%so as not to confuse
%We can use it  to get the empirical
%covariance matrix---i.e.~asymptotic approximation of the covariance matrix---of $\beta^{\ast}_{est}$.
 %for the estimator determined

 %From
%boostrapping---a powerful tool for approximating an estimator's bias and
%standard error in a statistical model---
%Using bootstrapping, we learn the empirical covariance
%matrix. 
%This provides us information about the possible correlation between the players'
%parameter estimations and thus, their behaviors. 
%%In particular, these
%%correlations reveal how players behaviors are correlated. 
 We
refer to the learned utility---$\hat{f}_{i}$ for player $i$---from the robust utility learning framework as the
nominal utility. The estimated nominal utility function for player $i$
%using one of the proposed batch methods 
is given by
\begin{equation}
  \hat{f}_{i}(x_i, x_{-i})=\psi_i(x_i,
x_{-i})+\hat{\theta}_{i}^\ast\phi_i(x_i, x_{-i})
  \label{eq:nominal}
\end{equation}
where $\hat{\theta}_i^\ast$ is extracted
from 
$\beta_{i,est}^\ast=(\hat{\mu}_i^{1\ast},
\hat{\mu}_i^{2\ast}, \hat{\theta}_i^\ast)$ which represents our estimate using one of the batch methods.
%in which we learn a utility
%function for the users that combines a players nominal  who are correlated with each. and try to re-estimate their utility functions assuming that they play under a correlated game. 

Using the correlations we learn when we estimate $\hat{f}_{i}$, we
construct a new utility $\hat{g}_{i}$ by combining scaled versions of a subset
(potentially all) of
the other
agents' utilities that are correlated with agent $i$. Let $\mc{Q}_i\subset
\mc{I}$ denote the
subset of agents correlated with agent $i$ and let $\mc{K}_i\subset\mc{Q}_i$ be
the set of agents used in constructing $\hat{g}_i$.
The correlated utility $\hat{g}_i$ for player $i$ is given by 
\begin{align}
  \hat{g}_{i}(x_i,x_{-i}) %&=\sum_{j\in \mc{Q}_i}\frac{\alpha_{i,j}}{c_{i,j}}\hat{f}_{i,}(x_i,x_{-i})\\
  &=\sum_{j\in
  \mc{K}_i}\frac{\alpha_{i,j}}{c_{i,j}}\psi_i(x_i,x_{-i})+\alpha_{i,j}\hat{\theta}_j^\ast\phi_i(x_i,x_{-i})
   %\hat{f}_{i,\text{nom}}(x_i,x_{-i})
  \label{eq:corest-1}
\end{align}
%where $\mc{Q}_i\subset \{1, \ldots, \np\}$ is the subset of players correlated
%with player $i$,
%\begin{multline}\label{eq:correlatedutility}
%  f_{j, \text{cor}}(x_j, x_{-j}) = \frac{\alpha_{j,j}}{c_1} \psi_j(x_j, x_{-j}) + \sum_{z=1, z \neq j}^{m} \frac{\alpha_{z,j}}{c_1} \psi_j(x_j, x_{-j}) \\ + \frac{\alpha_{j,j}}{c_2} \theta_{j} \phi_j(x_j, x_{-j}) + \sum_{z=1, z \neq j}^{m} \frac{\alpha_{z,j} }{c_2} \theta_{z} \phi_j(x_j, x_{-j}) = \\
%\frac{\alpha_{j,j} + \sum_{z=1, z \neq j}^{m} \alpha_{z,j} }{c_1} \psi_j(x_j, x_{-j}) + \frac{\alpha_{j,j} \theta_{j} + \sum_{z=1, z \neq j}^{m} \alpha_{z,j} \theta_{z} }{c_2} \\ \phi_j(x_j, x_{-j}) = 
%\hat{w}_j \psi_j(x_j, x_{-j}) + \hat{\theta}_{j}\phi_j(x_j, x_{-j})
%\end{multline}
%
%where 
%$\hat{w}_j = \frac{\alpha_{j,j} + \sum_{z=1, z \neq j}^{m} \alpha_{z,j} }{c_1}$, $\hat{\theta}_{j} = \frac{\alpha_{j,j} \theta_{j} + \sum_{z=1, z \neq j}^{m} \alpha_{z,j} \theta_{z} }{c_2}$, 
where $\alpha_{i,i}$ is the estimated variance of player $i$  determined by the empirical
covariance matrix, $\alpha_{i,j}$ is the covariance between the parameter
estimates for player $i$ and $j$
also determined by the empirical covariance matrix, and $c_{i,j}$ are scaling
constants.
We refer to the resulting game as an \emph{approximated correlation game}\footnote{We remark that there exists an equilibrium concept called \emph{correlated
equilibrium}~\cite{aumann:1974aa} which generalizes a Nash
equilibrium by characterizing correlations between randomized strategies; we
mention this only to alleviate  any potential confusion. 
The equilibrium concept we utilize for the
approximated correlation game is still a pure Nash equilibrium and there is no
coordinating mechanism.}.


%We apply two different methods for assembling the correlated utilities.
%This formally means that having a set of $\np$ users, with 
 
%Player $j$ under a correlated game has a re-estimated utility function $F_j$ as follows
%We try two] different forms of the correlated utilities. 
%The first construction of the 
%Our goal is to select these scaling constants in order to
%reduce the forecasting error.

%The re-estimated utility function under correlated game $F_j$  has an exact similar form as the utility estimated using batch methods $f_j$ . However, one critical difference is on the fact that now we introduce $\hat{w}_j $ and $\hat{\theta}_{j}$, which take in account the high correlation between some players' actions - profiles. It seems natural that some players have highly correlated actions - profiles and their actions influence each other. Our proposed utility learning algorithm under a correlated game can be described in two steps: First, we estimate users utility functions using cOLS and the proposed robust batch methods. Then, using a grid search we tune parameters $c_1, c_2$ by choosing those that minimize the forecasting error (Root Mean Square Error) on the training set. This gives us re-estimated utility functions as \eqref{eq:correlatedutility} that capture the correlated game between players and are able to give a better forecasting accuracy. 

%We refer to the game with correlated utilities as a \emph{psuedo--coalitional
%game} since it captures how players are potentially forming coalitions and
%collaborating. In fact, it captures what are essentially \emph{anti-coalitions}

%The second construction of $\hat{g}_i$ is given by
%\begin{align}
%  \hat{g}_{i}(x_i,x_{-i})&=\sum_{j\in \mc{Q}_i}\frac{\alpha_{i,j}}{c_{i,j}}\hat{f}_{j,}(x_j,x_{-j})\\
%   &=\sum_{j\in \mc{Q}_i}\frac{\alpha_{i,j}}{c_{i,j}}\big(\psi_j(x_j,x_{-j})+\hat{\theta}_j\phi_j(x_j,x_{-j})\big)
%  \label{eq:corest-2}
%\end{align}
%The difference is the fact that for player $i$, instead of weighting only her
%utility function in the construction of $\hat{g}_i$, we now taked a weighted sum of
%the utilities of all players correlated with player $i$. 
%
Given the form of $\hat{g}_i$, our goal is to select the scaling
constants $c_{i,j}$ in order to
reduce the forecasting error. Using our training data, we
formulate a convex optimization problem using the first-- and second--order
conditions on each agent's individual optimization problem where we assume that
agent $i$ is optimizing $\hat{g}_i$: %which is given by
\begin{equation}
  \max_{x_i\in [0,100]}\hat{g}_i(x_i,x_{-i}).
  \label{eq:indmin}
\end{equation}
The convex optimization problem we solve is formulated in a similar fashion to % how we fomulate
the base utility learning problem of Section~\ref{sec:baseutility}. 


In particular, we
solve a convex optimization problem formulated as follows. Define the vector $z_i\in \mb{R}^{|\mc{K}_i|}$ by
\begin{equation}
  z_i=\left[ {c_{i,j}}^{-1} \right]_{j\in \mc{K}_i}.
  \label{eq:z-c}
\end{equation}
and let 
\begin{equation}
  z=\left( c_{1,1}^{-1}, c_{1,2}^{-1}, \ldots, c_{1,
|\mc{K}_1|}^{-1}, \ldots, c_{\np, 1}^{-1},
\cdots, c_{\np, |\mc{K}_\np|}^{-1}\right).
  \label{eq:ztot}
\end{equation}
For agent $i$'s
optimization problem~\eqref{eq:indmin}, let the residual of the stationarity
condition be given by 
%\begin{subequations}
 \begin{align}
  \label{eq:dstatzero-1}
  \textstyle  r_{\text{s},i}^{(k)}(z_i, \mu_i;\hat{\theta}^\ast) &= \textstyle D_i\hat{g}_i(x_i^{(k)},
  x_{-i}^{(k)})+\sum_{j=1}^2\mu_i^{j}D_ih_{i,j}(x_i^{(k)})
\end{align}
and the residual of the complementary conditions be given by
\begin{align}
  r_{\text{c},i}^{j,(k)}(\mu_i) &=  \mu_i^{j}h_{i,j}(x_i^{(k)}), \ j\in \{1,2\}.
\label{eq:dslaczero-1}
\end{align} 
As before, let
$r_{\text{c},i}^{(k)}(\mu_i)=[r_{\text{c},i}^{1,(k)}(\mu_i)\
r_{\text{c},i}^{2,(k)}(\mu_i)]$.
Define $Q_i\in \mb{R}^{n_i\times|\mc{K}_i|}$ 
%for each $i\in\{1,\ldots,
%\np\}$ 
by
\begin{align}
  Q_i=\left[ \alpha_{i,j}D_{i,i}^2\psi_i(x^{(k)}) \right]_{k=1,j\in\mc{K}_i}^{n_i}.
  \label{eq:meth1Q}
\end{align}
and $q_i\in \mb{R}^{n_i}$ by
\begin{equation}
  q_i=\left[ \sum_{j\in \mc{K}_i}\hat{\theta}^{\ast}_j\alpha_{i,j}D_{i,i}^2\phi_i(x^{(k)})
  \right]_{k=1}^{n_i}.
  \label{eq:vector1}
\end{equation}
%\begin{equation}
%  q_i=[-\alpha_{i,j}\hat{\theta}_i
%  D_{i,i}^2\phi_i(x^{(k)})]
%  \label{<++>}
%\end{equation}<++>
%and
%\begin{align}
%  Q_i^2=\left[ \alpha_{i,j}(D_{i,i}^2\psi_j(x^{(k)})+\hat{\theta}_j
%  D_{i,i}^2\phi_j(x^{(k)}) \right]_{k=1,j\in\mc{Q}_i}^{n_i}.
%  \label{eq:meth1Q}
%\end{align}
Then,  we have the following convex optimization problem:
\begin{equation}
 \begin{aligned}
   &   \min\limits_{z,\mu}\sum_{i=1}^p
   \sum_{k=1}^{n_i}\chi(r_{\text{s},i}^{(k)}(z_i, \mu_i; \hat{\theta}^\ast),
  r_{\text{c},i}^{(k)}(\mu_i))\\
  %\bigg|\ 
  &  \text{s.t.}\ \ Q_iz_i+q_i\leq 0,  \ \mu_i\geq 0\  \ \forall \ i\in \mc{I}
  %-\frac{\alpha_{i,j}}{c_{i,j}}\left( 1+\hat{\theta}_j \right)
  %\geq c_{\LB}, \ \text{for each } i \text{ and } \forall j\in
  %\mc{Q}_i\\
  %&\quad \mu_i\geq 0, \text{ for each } i
\end{aligned}
\tag{P'}\label{opt-Pprime}
\end{equation}
Solving \ref{opt-Pprime} gives us estimated correlated utilities $\hat{g}_i$ for
each $i\in \mc{I}$ that we then use to forecast the agents' decisions.
%where $z=\left( c_{1,1}^{-1}, c_{1,2}^{-1}, \ldots, c_{1,
%|\mc{Q}_1|}^{-1}, \ldots, c_{\np, 1}^{-1},
%\cdots, c_{\np, |\mc{Q}_\np|}^{-1}\right)$.
%$c=(c_{1,1}, c_{1,2}, \ldots, c_{1,|\mc{Q}_1|}, \ldots, c_{\np, 1},
%\cdots, c_{\np, |\mc{Q}_\np|})$.
%\textcolor{blue}{If players are anti-correlated, the bound translates to
%$c_{i,j}<0$, if players are correlated (correlation positive) then the bound is
%just $c_{i,j}>0$ regardless of $\theta$ and the number of players}
%\begin{align}
%  &[\alpha_{i,1}(D_{i,i}^2\psi_1(x^{(k)})+\hat{\theta}_1 D_{i,i}^2\phi_1(x^{(k)})\\
%  &\cdots \
%  \alpha_{i,\np}(D_{i,i}^2\psi_{\np}(x^{(k)})+\hat{\theta}_\np
%  D_{i,i}^2\phi_{\np}(x^{(k)})]
%  \label{eq:bound}
%\end{align}

%In
%particular, we solve 
%%utility we now use each player
%Let 
%\[Q=D_{i}\Phi_i(x)\]
%\] %+\alpha_{1,3}f_3(x_3,x_{-3})\]
%\[f_{corr,1}(x_1,x_{-1})=
%\frac{\alpha_{1,1}}{c_{1,1}}(\phi(x_1,x_{-1})+\theta_1\psi(x_1,x_{-1}))+\frac{\alpha_{1,2}}{c_{1,2}}(\phi(x_2,x_{-2})+\theta_2\psi(x_2,x_{-2}))\]
%\[f_{corr,2}(x_2,x_{-2})=
%\frac{\alpha_{2,1}}{c_{2,1}}(\phi(x_1,x_{-1})+\theta_1\psi(x_1,x_{-1}))+\frac{\alpha_{2,2}}{c_{2,2}}(\phi(x_2,x_{-2})+\theta_2\psi(x_2,x_{-2}))\]
%for each iteration in your grid search,
%select 
%\[c=(c_{1,1},c_{1,2},c_{2,1},c_{2,2})\]
%compute Nash. Save the value and then repeat over your whole grid.



